Offline Equilibrium Finding

Offline reinforcement learning (offline RL) is an emerging field that has recently begun gaining attention across various application domains due to its ability to learn strategies from earlier collected datasets. Offline RL proved very successful, paving a path to solving previously intractable real-world problems, and we aim to generalize this paradigm to a multiplayer-game setting. To this end, we introduce a problem of offline equilibrium finding (OEF) and construct multiple types of datasets across a wide range of games using several established methods. To solve the OEF problem, we design a model-based framework that can directly apply any online equilibrium finding algorithm to the OEF setting while making minimal changes. The three most prominent contemporary online equilibrium finding algorithms are adapted to the context of OEF, creating three model-based variants: OEF-PSRO and OEF-CFR, which generalize the widely-used algorithms PSRO and Deep CFR to compute Nash equilibria (NEs), and OEF-JPSRO, which generalizes the JPSRO to calculate (Coarse) Correlated equilibria ((C)CEs). We also combine the behavior cloning policy with the model-based policy to further improve the performance and provide a theoretical guarantee of the solution quality. Extensive experimental results demonstrate the superiority of our approach over offline RL algorithms and the importance of using model-based methods for OEF problems. We hope our work will contribute to advancing research in large-scale equilibrium finding.

==> paper_files/oef_benchmark.tex <==

\section{Algorithms for Offline Equilibrium Finding}

In real life, the offline dataset may be collected using an unknown behavior strategy. To simulate real-world cases, we focus on four types of datasets: expert dataset, learning dataset, random dataset, and hybrid dataset. Based on the offline datasets, we give the formal definition of the offline equilibrium finding problem. Details of offline datasets, the relationship between the information set $I$ and game state $s_t$ can be found in Appendix~\ref{app:dateset}.
\begin{definition}[OEF]
Given a game's offline dataset $\mathcal{D} = (s_t, a, s_{t+1}, r_{t+1})$ where $s_t$ and $s_{t+1}$ refer to the game state, $a$ refer to the action played at $s_t$ and $r_{t+1}$ refer to the reward after performing action $a$ at $s_t$. The strategy used to collect the dataset $\mathcal{D}$ is unknown. The OEF problem is to find an approximate equilibrium strategy profile $\sigma^*$ that achieves a small gap between $\sigma^*$ and equilibrium, i.e., the $\textsc{NashConv}$ for NE and (C)CE Gap Sum for (C)CE, only based on $\mathcal{D}$. 
\end{definition}
Then, we introduce our proposed model-based method (MB) for solving the OEF problem, which can adapt any online equilibrium finding algorithm into the context of the offline setting. Since the behavior cloning (BC) technique can learn a good policy when the behavior policy of the dataset is close to the equilibrium policy, which makes up for the deficiency of the model-based algorithm in this aspect, we apply the BC technique to further improve the performance of the model-based algorithm. To do this, we combine these two methods (BC+MB) by assigning different weights to trained policies using these two methods to get the final strategy (see the experiments for details). 

\begin{algorithm}[t]
\caption{General Framework of OEF}
\label{oef}
\begin{algorithmic}[1]
\STATE {\bfseries Input:} an offline dataset $D$
\STATE Train an environment model $E$ based on $D$;
\STATE Train a policy ${\pi}^{mb}$ on $E$ using OEF-PSRO/OEF-CFR;
\STATE Train a policy ${\pi}^{bc}$ based on $D$ using BC technique;
\STATE Combine ${\pi}^{bc}$ and ${\pi}^{mb}$ with weights $\alpha$ to get policy ${\pi}$;
\STATE {\bfseries Output:} a policy $\pi$
\end{algorithmic}
\end{algorithm}

\begin{figure}[t]
\centering
\includegraphics[width=0.6\linewidth]{figures/oef_flow.pdf}
\caption{The flow of OEF algorithms.}
\label{fig:oef_flow}
\end{figure}

% a combination of the behavior cloning (BC) and model-based (MB) methods. Note that BC and MB are obvious choices for OEF. However, both BC and MB methods exhibit various flaws under different circumstances. Therefore, to avoid their drawbacks, we combine these two methods by assigning different weights to the trained policies using these two methods (see the experiments part for details). 

Figure~\ref{fig:oef_flow} and Algorithm \ref{oef} show the general procedure of the OEF algorithm. Given the offline dataset, we first train an environment model $E$ based on these game data. Then we perform an equilibrium finding algorithm on the trained environment model to learn a model-based policy (MB policy). To further improve the performance, we adopt the behavior cloning technique to learn a policy (BC policy) directly from the offline dataset. Then we combine these two policies, i.e., the BC policy and the MB policy, by assigning proper weights to these two policies to obtain the final policy under different cases. Here, we also provide the guarantee of the solution quality for our algorithm BC+MB. 
\begin{theorem}
Assuming that the environment model and the behavior cloning policy are well-trained, under the offline dataset $\mathcal{D}_{\sigma}$ generated using $\sigma$, BC+MB can get the strategy which is at least as good as $\sigma$. If the offline dataset $\mathcal{D}_{\sigma}$ covers $(s_t, a, s_{t+1}), \forall s_t, a \in A(s_t)$, BC+MB can get an equal or better strategy than $\sigma$.
\end{theorem}
The proof of the theorem and more analysis about the relationship between the dataset coverage and our algorithm can be found in Appendix~\ref{app:theoretical}. We leave two unexplored options for future research: i) whether we can learn an MB policy with the regularization of the BC policy, as well as interacting with the dataset, and ii) if we can use the learned model to get the proper weights when combining the two policies. Next, we move to introduce the details of our model-based method. The details of the behavior cloning technique can be found in Appendix~\ref{app:implementation}.

\subsection{Environment Model}
In the OEF setting, a relationship between an equilibrium strategy and an offline dataset is needed. To compute the equilibrium strategy  based on the offline dataset, we cannot use the data of two action tuples to determine which action tuple is closer to an equilibrium strategy since the equilibrium identification requires other action tuples to serve as references~\cite{cui2022offline}. For computing equilibrium strategies, we hence need to be able to evaluate any action tuple, and the data of some may be missing from the dataset. It prevents us from using model-free methods to learn the equilibrium strategy from the dataset directly which also means that we cannot build a direct relationship between the equilibrium strategy and the offline dataset. Therefore, model-based methods, rather than other model-free methods, are arguably the most appropriate choices for solving the OEF problem. Unfortunately, most known model-based methods for single-agent RL cannot be directly applied to games for equilibrium findings. The main reason is their inherent reliance on the existence of no strategic opponents in the environment. To this end, we propose to introduce an environment model as the intermediary between the equilibrium strategy and the offline dataset. 
From the above analysis, to compute the equilibrium strategy, we need to be able to evaluate any action tuple. Therefore, the trained environment model needs to be able to capture the game information which is necessary for evaluating any action tuple. In other words, the trained environment model needs to be able to output the next game state information (state, rewards, etc) conditional to the current game state and action. Here, we take the deep neural network as the environment model due to its powerful generalization abilities. Therefore, the deep neural network model can provide approximate results for game states not sufficiently captured in the data. 

Then we move to introduce how to train an environment model based on an OEF dataset. Figure \ref{fig:mb_model} shows the structure of the environment model. The environment model $E$ parameterized by $\theta_e$ takes the game state $s_t$ and action $a$ of the player, who played at the state $s_t$, as inputs and outputs the next game state $s_{t+1}$, the rewards $r_{t+1}$ of all players, and other information such as the next legal action set and whether the game ends. To deal with the chance player in the game, we also predict whether the next state is a chance node or not, and if the next state is a chance node, then we sample an action according to the predicted legal action set to play. We take the stochastic gradient descent (SGD) as the optimizer to perform parameter updates. Any loss function that satisfies the conditions of Bregman divergence \citep{banerjee2005clustering} can be employed. Here, we use the mean squared error loss which can be defined as below:
\begin{figure}[t]
    \centering
\includegraphics[width=0.7\linewidth]{figures/mb_model.pdf}
    \caption{Environment model structure.}
    \label{fig:mb_model}
\end{figure}
\begin{align}
    \mathcal{L}_{env} &= \mathbb{E}_{D} [MSE((s_{t+1}, r_{t+1}), E(s_t, a;\theta_e))] \nonumber. 
\end{align}
Finally, we train the environment model by performing mini-batch SGD iterations. 

\subsection{Model-Based Algorithms}
Once the environment model is well-trained, the model can provide enough game information for equilibrium computation. To compute the equilibrium strategy based on the environment model, we generalize existing online equilibrium finding algorithms to the context of the OEF setting by replacing the actual environment with the well-trained environment model. In this paper, we propose three model-based algorithms: Offline Equilibrium Finding-Policy Space Response Oracles (OEF-PSRO) and Offline Equilibrium Finding-Deep CFR (OEF-CFR) algorithms, which generalize PSRO and Deep CFR to compute NEs, and Offline Equilibrium Finding-Joint Policy Space Response Oracles (OEF-JPSRO), which generalize JPSRO to compute (C)CEs. Then we move to introduce these algorithms in detail.

In PSRO or JPSRO, a meta-game is represented as an empirical game starting with a single policy (uniform random) and iteratively enlarged by adding new policies (oracles) that approximate the best responses to the meta-strategies of other players. It is clear that when computing the best response policy oracle, interactions with the environment are required to gain game information. In the OEF setting, only an offline dataset is provided, and directly applying PSRO or JPSRO is not feasible. In OEF-PSRO and OEF-JPSRO, we use the trained environment model to replace the actual environment to provide the game information. It is common knowledge that when computing the best response policy using DQN or other RL algorithms, the next state and reward based on the current state and the action are required. Our environment model can provide such information. The model can also offer additional information for approximating the missing entries in the meta-game matrix using the same manner. 
Deep CFR is a variant of CFR that uses neural networks to approximate counterfactual regret values and average strategies. During this approximation, the game tree has to be partially traversed to arrive at the counterfactual regret value. This process requires an environment to provide the necessary game information. Akin to OEF-PSRO, also in OEF-CFR, we use the trained environment model to replace the actual environment. During the traversal, the environment needs to identify the next game state and utility for the terminal game state, for which we employ our trained environment model. These algorithms are described in detail in Appendix~\ref{app:implementation}.

We also provide a minimal dataset coverage assumption for the model-based algorithm to converge to the NE strategy of the underlying game in the OEF setting. 
The proof and more discussion about the performance of our OEF algorithm on the different datasets can be found in Appendix \ref{app:theoretical}.
\begin{assumption} (Uniform Coverage)
    For all state $s_t$ and all actions $a_t \in A(s_t)$, all state-action pairs $(s_t, a_t, s_{t+1})$ are covered by the dataset. 
\end{assumption}

==> paper_files/oef_datasets.tex <==

\section{Datasets for Offline Equilibrium Finding}
\label{sec:dataset}
In the offline setting, a fixed pre-collected dataset is provided, and the goal is to compute NE using the dataset only. In the real life, offline datasets may be collected using different behavior strategies. In this paper, to simulate real-world cases, we focus on the following three types of datasets.
% \textcolor{red}{Describe the game and the collecting methods. }
% TODO: give more detail information about dataset

\textbf{Random dataset.} This type of dataset is collected using a random strategy. The motivation behind this is that when we do not know how to play a game, we may try to explore it randomly. The process of collecting is akin to that of a beginner familiarizing themselves with the game for the first time. The dataset is collected in three steps. First, we assume that every player plays a uniform strategy. Second, the players engage in the game repeatedly. Finally, we collect the generated game data. Note that in imperfect-information extensive-form games, the definition of information sets corresponds to the decision points of players. Here, we take the information sets of all players in the game as a game state. Therefore, the game data include the transition information such as current game state $s_t = (I^t_1, I^t_2, ..., I^t_n)$, action $a$, next game state $s_{t+1} = (I^{t+1}_1, I^{t+1}_2, ..., I^{t+1}_n)$, and other game information, e.g., whether the game ends and players' rewards $r_{t+1} = (r^{t+1}_1, r_2^{t+1}, ..., r_n^{t+1})$. 

\textbf{Learning dataset.} This type of dataset is collected when learning the Nash equilibrium strategy. When solving a game using some existing equilibrium finding algorithm, the players have to interact with the game environment. During the course of learning, we may gather these intermediate interaction game data and store them as a learning dataset. In contrast to the random dataset, the players' strategies gradually improve as we get closer to Nash equilibrium.   

\textbf{Expert dataset.} This type of dataset is collected using an NE strategy. The motivation behind the dataset is that when learning a game, we often prefer to observe more experienced players at play. We simulate the expert players using the NE strategy and collect the interaction data. We follow a similar methodology as with the random dataset. First, we compute the NE strategies using any existing equilibrium finding algorithm. As a second step, the Nashian players repeatedly interact in the game. Finally, we gather the generated data and store them as the expert dataset. 

In addition to the three types of datasets mentioned above, we also consider hybrid datasets consisting of random and expert interactions mixed in different ratios to simulate offline datasets generated by unknown strategies. We collect the data from player engagements in the most frequently used benchmarking imperfect-information extensive-form games in contemporary research on equilibrium finding. These games include poker games (two-player and multi-player Kuhn poker, two-player and multi-player Leduc poker), Phantom Tic-Tac-Toe, and Liar's Dice. 


==> paper_files/oef_experiments.tex <==

\section{Experiments}\label{sec:experiments}
Finally, in this section, we present the benchmark results of the OEF algorithms on the OEF datasets collected in various games. First, we evaluate the behavior cloning method and the model-based method on different datasets independently. Then, we move to assess the performance of our benchmark algorithms (BC+MB), a combination of both methods described in the previous section. 

\subsection{Experimental Setting}\label{sec:experiments_setting}
OpenSpiel~\footnote{\url{https://github.com/deepmind/open_spiel}} is a collection of environments and algorithms for research in general reinforcement learning and search/planning in games \citep{lanctot2019openspiel}. It is widely accepted and implements many different games. We use it as our experimental platform and select several poker games as experimental domains. We opt for Kuhn poker, Leduc poker, Phantom Tic-Tac-Toe, and Liar's Dice, which are all widely used in previous works~\citep{lisy2015online,brown2019solving}. % experimental process
For every game, we first generate the three datasets introduced in Section \ref{sec:dataset}. Then we mix the random dataset and the expert dataset in different proportions to get hybrid datasets. Based on these hybrid datasets, we first train the behavior cloning strategies using imitation learning. Then we train the environment model by performing mini-batch stochastic gradient descent (SGD) iterations. After obtaining the environment model, we employ it in the OEF-PSRO and OEF-CFR algorithms to compute the Nash equilibrium strategy. Finally, we combine the BC policy and the MB policy to obtain the final policy. We use NashConv (exploitability) as the optimality measure. 
% computer setting
All the experiments are performed on a server with a 10-core 3.3GHz Intel i9-9820X CPU and an NVIDIA RTX 2080 Ti GPU. All results are averaged over three seeds. Only selected results are shown here and the rest is deferred to Appendix C.

\subsection{Two Player Games}



% \subsection{Performance of the Behavior Cloning Method}

\begin{figure}[t]
\centering
\subfigure[Dataset Analysis]{
\includegraphics[width=0.235\textwidth]{iclr2023/figures/results/kuhn_poker/kuhn_poker_2_player_fft_2.pdf}}
\subfigure[Offline RL]{
\includegraphics[width=0.235\textwidth]{iclr2023/figures/results/kuhn_poker/kuhn_poker_2_players_offline_rl.pdf}}
\subfigure[Behavior Cloning]{
\includegraphics[width=0.235\textwidth]{iclr2023/figures/results/kuhn_poker/kuhn_poker_2_players_bc.pdf}}
\subfigure[Model Based Method]{
\includegraphics[width=0.235\textwidth]{iclr2023/figures/results/kuhn_poker/kuhn_poker_2_players_mb.pdf}}
\subfigure[BC+MB]{
\includegraphics[width=0.235\textwidth]{iclr2023/figures/results/kuhn_poker/kuhn_poker_2_players_bc_mb_500.pdf}}
\subfigure[BC+MB]{
\includegraphics[width=0.235\textwidth]{iclr2023/figures/results/kuhn_poker/kuhn_poker_2_players_bc_mb_1000.pdf}}
\subfigure[Weight]{
\includegraphics[width=0.235\textwidth]{iclr2023/figures/results/kuhn_poker/kuhn_poker_2_players_min_weight_2.pdf}}
\subfigure[Learning Dataset]{
\includegraphics[width=0.235\textwidth]{iclr2023/figures/results/kuhn_poker/kuhn_poker_players_learning_dataset.pdf}}
\caption{Experimental Results on Two-Player Kuhn Poker.}
\end{figure}

\begin{figure}[t]
\centering
\subfigure[Dataset Analysis]{
\includegraphics[width=0.23\textwidth]{iclr2023/figures/results/leduc_poker/leduc_poker_2_player_fft_2.pdf}}
\subfigure[Offline RL]{
\includegraphics[width=0.23\textwidth]{iclr2023/figures/results/leduc_poker/leduc_poker_2_players_offline_rl.pdf}}
\subfigure[Behavior Cloning]{
\includegraphics[width=0.235\textwidth]{iclr2023/figures/results/leduc_poker/leduc_poker_2_players_bc.pdf}}
\subfigure[Model Based Method]{
\includegraphics[width=0.235\textwidth]{iclr2023/figures/results/leduc_poker/leduc_poker_2_players_mb.pdf}}
\subfigure[BC+MB]{
\includegraphics[width=0.235\textwidth]{iclr2023/figures/results/leduc_poker/leduc_poker_2_players_bc_mb_10000.pdf}}
\subfigure[BC+MB]{
\includegraphics[width=0.235\textwidth]{iclr2023/figures/results/leduc_poker/leduc_poker_2_players_bc_mb_20000.pdf}}
\subfigure[Weight]{
\includegraphics[width=0.235\textwidth]{iclr2023/figures/results/leduc_poker/leduc_poker_2_players_min_weight_2.pdf}}
\subfigure[Learning Dataset]{
\includegraphics[width=0.235\textwidth]{iclr2023/figures/results/leduc_poker/leduc_poker_players_learning_dataset.pdf}}
\caption{Experimental Results on Two-Player Leduc Poker.}
\end{figure}

We first evaluate the performance of the behavior cloning technique in the OEF. We apply the behavior cloning technique to learn the BC policy for every player on every hybrid dataset and compute the NashConv of these BC policies. Figures show the results of Kuhn pokers with a different number of players. The x-axis represents the proportion of random data in the hybrid dataset. If the proportion is zero, the mixed dataset equals the expert dataset. If the proportion is one, it indicates that the hybrid dataset is the random dataset. We can see that as the proportion of random dataset increases, the performance of BC policy decreases in all games. The finding is intuitive since the BC method only performs better on datasets containing more expert data. We also test the BC method in several datasets of different sizes. With the increase in the dataset size, the performance evolves more stable while the performance improvement is not very significant. Therefore, the performance of BC policy depends on the quality of datasets, i.e., the quality of the policy used to generate the dataset.

\subsection{Multi-player Games}
% \subsection{Performance of the Model-based Methods}
\begin{figure}[t]
\centering
\subfigure[Dataset Analysis]{
\includegraphics[width=0.23\textwidth]{iclr2023/figures/results/kuhn_poker/kuhn_poker_3_player_fft_2.pdf}}
\subfigure[OEF-JPSRO]{
\includegraphics[width=0.23\textwidth]{iclr2023/figures/results/kuhn_poker/kuhn_poker_3_players_jpsro.pdf}}
\subfigure[Dataset Analysis]{
\includegraphics[width=0.23\textwidth]{iclr2023/figures/results/kuhn_poker/kuhn_poker_3_player_fft_2.pdf}}
\subfigure[OEF-JPSRO]{
\includegraphics[width=0.23\textwidth]{iclr2023/figures/results/kuhn_poker/kuhn_poker_3_players_jpsro.pdf}}

\caption{Experimental Results on Multi-Player Games.}
\end{figure}
Here, we evaluate the performance of the model-based algorithm in the OEF. 
% The test process is similar to the process of testing the behavior cloning technique. 
For every hybrid dataset, we first train an environment model. Then we perform OEF-CFR or OEF-PSRO algorithms on the trained environment model to learn the NE strategy as the MB policy. Finally, we compute the NashConv to evaluate the MB policy. Figures show the results of the model-based algorithm in Kuhn poker with a different number of players. From Figure , we find that OEF-CFR and OEF-PSRO can get almost the same results. It indicates that the performance of MB mainly depends on the quality of the trained environment model, and we can use either algorithm to calculate MB policy. We find that with the increase in the dataset size, the performance becomes better. It indicates that if the dataset includes enough data, the trained environment model is closer to the actual environment (test environment). Though with the increase of the proportion of random datasets, the performance of MB policy becomes better, the improvement is not very significant, and the trend is almost gone when the number of players is large. Therefore, the performance of MB policy mainly depends on the size of datasets and is mildly influenced by the quality of datasets. We noticed that the MB method performed worse in games with more players than in games with fewer players. It indicates that OEF in multi-player games is more challenging than in two-player games.
% since there are more uncertain factors in multi-player games.
% The dynamics in these multi-player games may be the main reason and it  
% It indicates that OEF in multi-player games is more challenging than in two-player games since there are more uncertain in multi-player games.
% With the increase of the proportion of random datasets, the performance of MB method becomes better. It indicates that if the dataset includes more random data, then the trained environment model is closer to the real environment. Another finding is that 
% With the increase of the size of the dataset, the performance becomes better. These findings are in line with intuition. In other words, if the dataset includes enough data, then the trained environment model can provide enough information for equilibrium finding algorithms and good information which is close to the real environment. Therefore the performance of MB policy mainly depends on the size of datasets and is mildly influenced by the quality of datasets.
% From results in kuhn poker with different player numbers, when there are more players, the performance of the MB policy becomes worse. It may be caused by the high dynamics in these multi-player games. Therefore, OEF in multi-player games is more challenging.

\subsection{Performance of the Benchmark Algorithm BC+MB}
% Given an offline dataset, according to the above process, we can get a BC policy and an MB policy. 
From the above results, we find that the BC policy performs poorly in the random dataset while the performance of the MB method is good. However, the MB method performs poorly in the expert dataset, while the BC policy can perform well.
Therefore, to get a better policy on the dataset generated by an unknown strategy, a straightforward way is to merge these two policies by assigning proper weights to them in different cases. Here, we use a simple merging method to combine these two policies. Let $\alpha$ be the weight of BC policy. Then the weight of the MB policy is $1-\alpha$. We preset 11 weight assignment plans, i.e., $\alpha\in\{0, 0.1, 0.2, ..., 0.9, 1\}$. Next, we use these 11 weight assignment plans to combine these two policies to get a set of final policies. Then we test these final policies in a real game to get the best final policy. Another more complex method is to learn the weights using few-shot interactions with the real game. We left this as future work. 

% \begin{figure}[t]
% \centering
% \subfigure[Kuhn Poker-2 Player]{
% \includegraphics[width=0.235\textwidth]{figures/results/kuhn_poker/kuhn_poker_2_players_bc_mb_500_2.pdf}
% \label{kuhn_2}}
% \subfigure[Kuhn Poker-2 Player]{
% \includegraphics[width=0.235\textwidth]{figures/results/kuhn_poker/kuhn_poker_2_players_bc_mb_1000_2.pdf}}
% \subfigure[Leduc Poker-2 Player]{
% \includegraphics[width=0.235\textwidth]{figures/results/leduc_poker/leduc_poker_2_players_bc_mb_10000_2.pdf}}
% \subfigure[Leduc Poker-2 Player]{
% \includegraphics[width=0.235\textwidth]{figures/results/leduc_poker/leduc_poker_2_players_bc_mb_20000_2.pdf} \label{kuhn_5}}
% \subfigure[Kuhn Poker-2 Player]{
% \includegraphics[width=0.23\textwidth]{figures/results/kuhn_poker/kuhn_poker_2_players_min_weight_2.pdf}
% \label{weight_1}}
% \subfigure[Leduc Poker-2 Player]{
% \includegraphics[width=0.23\textwidth]{figures/results/leduc_poker/leduc_poker_2_players_min_weight_2.pdf}
% \label{weight_2}}
% \subfigure[Kuhn Poker]{
% \includegraphics[width=0.23\textwidth]{figures/results/kuhn_poker/kuhn_poker_players_learning_dataset.pdf}
% \label{learning_1}}
% \subfigure[Leduc Poker]{
% \includegraphics[width=0.23\textwidth]{figures/results/leduc_poker/leduc_poker_players_learning_dataset.pdf}
% \label{learning_2}}
% \caption{Experimental results of the benchmark algorithm BC+MB.}
% \label{fig:mb_bc}
% \end{figure}

Figures show the performance of the BC+MB method in Kuhn poker and Leduc poker under offline datasets with different sizes. The results of BC and MB methods are also plotted for comparison. We find that the BC+MB method performs better than both BC and MB methods in all cases. Figures show the weights of BC ($\alpha$) that make these combined policies perform best in these datasets. We find that as the proportion of the random dataset increases, the weight of the BC policy in the final policy decreases. It indicates that when the dataset includes many expert data, i.e., the proportion of random datasets is low, the performance of the BC policy is always better than the MB policy, whatever the size of the dataset. Therefore, in that case, the weight of the BC policy is high.
% We find that as the size of the dataset increases, the weight of the BC policy in the final policy decreases. As mentioned before, the performance of the BC policy mainly depends on the quality of the dataset while the performance of the MB policy mainly depends on the size of the dataset. It indicates that when the size of the offline dataset is small, the MB policy performs not well and the weight of the BC policy in the final policy is high. However, when the size of the offline dataset is big, the performance of the MB policy is much better than the BC policy. In this case, the weight of the BC policy in the final policy is very low. Note that when the dataset includes many expert data, i.e., the proportion of random datasets is low, the performance of the BC policy is always better than the MB policy whatever the size of the dataset. Therefore, in that case, the weight of the BC policy is high. 
In conclusion, the BC+MB method can take the best of both BC and MB methods and perform better than BC method and MB method. We also test the BC+MB algorithm in learning datasets which can be viewed as datasets produced by an unknown strategy, and the results are shown in Figures. We find that BC+MB performs best among these methods. It indicates that given a dataset generated by an unknown strategy, BC+MB can always get a good policy.

